Domain Adversarial Training for Mitigating Gender Bias in Speech-based Mental Health Detection

Speech-based AI models are emerging as powerful tools for detecting depression and the presence of Post-traumatic stress disorder (PTSD), offering a non-invasive and cost-effective way to assess mental health. However, these models often struggle with gender bias, which can lead to unfair and inaccurate predictions. In this study, our study addresses this issue by introducing a domain adversarial training approach that explicitly considers gender differences in speech-based depression and PTSD detection. Specifically, we treat different genders as distinct domains and integrate this information into a pretrained speech foundation model. We then validate its effectiveness on the E-DAIC dataset to assess its impact on performance. Experimental results show that our method notably improves detection performance, increasing the F1-score by up to 13.29 percentage points compared to the baseline. This highlights the importance of addressing demographic disparities in AI-driven mental health assessment.

==> 7-Ack.tex <==
\vspace{-3pt}
\section{Acknowledgements}
\vspace{-1pt}
%This work was supported by the Ministry of Employment and Labor and HRD Korea's K-Digital Platform project, and Institute of Information \& communications Technology Planning \& Evaluation (IITP) grant funded by the Korea government (MSIT) (No. 2019-0-00075, Artificial Intelligence Graduate School Program (KAIST), 10\% and No.2022-0-00641, XVoice: Multi-Modal Voice Meta Learning, 45\%), and by the MSIT (Ministry of Science and ICT), Korea, under the ITRC (Information Technology Research Center) support program (IITP-2023-2020-0-01808) supervised by the IITP, 45\%.
This research was supported by a grant of the Korea Health Technology R\&D Project through the Korea Health Industry Development Institute (KHIDI), funded by the Ministry of Health \& Welfare, Republic of Korea (grant number: HI22C1962), and by a grant of the Mental Health related Social Problem Solving Project, Ministry of Health \& Welfare, Republic of Korea(grant number: RS-2024-00403474), and by the Bio Industry Technology Development Program funded by the Ministry of Trade, Industry \& Energy (MOTIE, Korea) (Project Number: RS-2024-00431485), and by Brian Impact Foundation, a non-profit organization dedicated to the advancement of science and technology for all.

==> Tables/Table5.tex <==
\begin{table}[htbp]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lcccccccccc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{5}{c}{Male} & \multicolumn{4}{c}{Female} & \multirow{2}{*}{F1 Gender Avg} \\
        \cmidrule(lr){2-6} \cmidrule(lr){7-10}
        & F1 (ND) & F1 (D) & F1 Avg & F1 (NP) & F1 (P) & F1 (NP) & F1 (P) & F1 Avg \\
        \midrule
        \multicolumn{10}{l}{\textbf{Depressed - Fine-tuning}} \\
        wav2vec2  & 79.32 & 22.35 & 50.84 & 43.48 & 61.99 & 52.73 & 51.785 \\
        HuBERT    & 76.58 & 33.68 & 55.13 & 35.3  & 47.36 & 46.33 & 48.235 \\
        WavLM     & 82.28 & 28.43 & 55.36 & 40.09 & 35.75 & 37.92 & 46.64 \\
        \midrule
        \multicolumn{10}{l}{\textbf{Depressed - Domain Adaptation}} \\
        wav2vec2  & 89.24 & 25.65 & 57.45 & 47.41 & 63.84 & 55.63 & 56.54 \\
        HuBERT    & 81.38 & 36.81 & 58.16 & 44.16 & 48.14 & 41.15 & 51.31 \\
        WavLM     & 87.82 & 26.75 & 57.29 & 42.14 & 40.11 & 41.13 & 49.21 \\
        \midrule
        \multicolumn{10}{l}{\textbf{PTSD - Fine-tuning}} \\
        wav2vec2  & 76.03 & 48.46 & 62.25 & 56.03 & 39.78 & 47.91 & 55.08 \\
        HuBERT    & 70.34 & 55.88 & 63.11 & 48.25 & 46.30 & 50.10 & 51.835 \\
        WavLM     & 70.73 & 49.5  & 60.12 & 48.25 & 40.79 & 44.52 & 44.82 \\
        \midrule
        \multicolumn{10}{l}{\textbf{PTSD - Domain Adaptation}} \\
        wav2vec2  & 77.01 & 50.63 & 63.82 & 54.93 & 47.77 & 51.35 & 57.675 \\
        HuBERT    & 77.79 & 59.22 & 68.51 & 53.97 & 42.11 & 48.04 & 58.275 \\
        WavLM     & 70.25 & 50.52 & 60.52 & 55.22 & 41.85 & 48.54 & 54.53 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Performance comparison of different models on Depressed and PTSD classification tasks.}
    \label{tab:results}
\end{table}
